Graphene: A Context-Preserving Open Information Extraction System

We introduce Graphene, an Open IE system whose goal is to generate accurate, meaningful and complete propositions that may facilitate a variety of downstream semantic applications. For this purpose, we transform syntactically complex input sentences into clean, compact structures in the form of core facts and accompanying contexts, while identifying the rhetorical relations that hold between them in order to maintain their semantic relationship. In that way, we preserve the context of the relational tuples extracted from a source sentence, generating a novel lightweight semantic representation for Open IE that enhances the expressiveness of the extracted propositions.

==> figures/head_relation_extractor.tex <==
\begin{figure}[htbp]
\centering

\begin{minipage}{.6\textwidth}
\centering
\begin{tikzpicture}[level distance=1.2cm, every tree node/.style={align=center}]
\Tree [.{topmost S\1}
          \edge[roof, dotted]; {z_1}
          NP\1
          \edge[roof, dotted]; {z_2}
          [.VP
            \edge[roof, dotted]; {z_3}
            \edge[dashed] node[midway, right] {VP*};
            [
              \edge[roof, dotted]; {z_4}
              {NP $\vert$ PP $\vert$\\S $\vert$ SBAR\\x}
              \edge[roof, dotted]; {z_5}
            ]
            \edge[roof, dotted]; {z_6}
          ]
          \edge[roof, dotted]; {z_7}
        ] 
\end{tikzpicture}
\end{minipage}%
\begin{minipage}{.4\textwidth}
\centering
rel $\gets$ $z_3$ \conc $z_4$\\
arg1 $\gets$ NP'\\
arg2 $\gets$ x \conc $z_5$\\
\end{minipage}


\caption{Pattern for Graphene's default relation extraction baseline (the symbol "\conc" denotes concatenation).}
\label{fig:headRelationExtractor}
\end{figure}

==> figures/workflow.tex <==
\begin{figure}[htbp]
\centering

\begin{minipage}{0.4\textwidth}
\centering
Input-Document\\
\vspace{0.2cm}
\begin{tikzpicture}[scale=0.6, every node/.style={align=center, transform shape}]
\node[rectangle, solid, draw=black, text width=1.0*\linewidth, rounded corners=5pt]{
[...] Although the Treasury will announce details of the November refunding on Monday, \ul{it} will be delayed if Congress and President Bush fail to increase the Treasury's borrowing capacity. [...]
};
\end{tikzpicture}
\end{minipage}%

\vspace{0.2cm}
$\downarrow$
\vspace{0.2cm}

Framework for Open Relation Extraction\\
\vspace{0.2cm}

\begin{cminipage}{0.98\textwidth}
\centering
\begin{minipage}{0.2\textwidth}
\centering
Coreference-Resolution\\
\vspace{0.2cm}
\begin{tikzpicture}[scale=0.6, every node/.style={align=center, transform shape}]
\node[rectangle, solid, draw=black, text width=1.0*\linewidth, rounded corners=5pt]{
[...] Although the Treasury will announce details of the November refunding on Monday, \ul{the funding} will be delayed if Congress and President Bush fail to increase the Treasury's borrowing capacity. [...]
};
\end{tikzpicture}
\end{minipage}%
\hspace{0cm}
$\rightarrow$
\hspace{0cm}
\begin{minipage}{0.7\textwidth}
\centering
Transformation Stage\\
\vspace{0.2cm}
\begin{tikzpicture}[scale=0.5, level distance=2.4cm, sibling distance=0cm, every tree node/.style={align=center, transform shape}]
\Tree [
.\node[style={draw,rectangle}] {DOCUMENT-ROOT}; 
  \edge node[midway, right] {core}; [
      .\node [style={draw,rectangle}] {COORD\\\textit{Contrast}};
            \edge node[midway, left] {core}; [.\node(a)[label=below:TEMPORAL(on Monday)]{The Treasury will\\announce details of\\the November refunding.};]
            \edge node[midway, right] {core}; [
              .\node [style={draw,rectangle}] {SUBORD\\\textit{Condition}};
                \edge node[midway, left] {core}; [.\node(b){The funding\\will be delayed.};]
                \edge node[midway, right] {context}; [
                  .\node [style={draw,rectangle}] {COORD\\\textit{List}};
                    \edge node[midway, left] {core}; [.\node(c){Congress fail to\\increase the Treasury's\\borrowing capacity.};]
                    \edge node[midway, right] {core}; [.\node(d){President Bush fail to\\increase the Treasury's\\borrowing capacity.};]
                ]
            ]
        ]
    ]
]
\end{tikzpicture}
\end{minipage}%

\vspace{0.2cm}
\hspace{0cm}
$\rightarrow$
\hspace{0cm}
\begin{minipage}{0.9\textwidth}
\centering
Relation Extraction\\
\vspace{0.2cm}
\begin{tikzpicture}[scale=0.6, every node/.style={align=center, transform shape}]
    \node(A)[text width=0.6*\linewidth, label=below:TEMPORAL(on Monday)]{The Treasury will announce details [...]};
    \node(B)[below of=A, yshift=-1cm, text width=0.6*\linewidth]{The funding will be delayed.};
    \node(C)[below of=B, yshift=-0.5cm, text width=0.6*\linewidth]{Congress fail to increase [...]};
    \node(D)[below of=C, yshift=-0.5cm, text width=0.6*\linewidth]{President Bush fail to increase [...]};

    \node(a)[right=1 of A, text width=0.6*\linewidth,  label=below:TEMPORAL(on Monday)]{\texttuple{The Treasury}{will announce}{details [...]}};
    \node(b)[right=1 of B, text width=0.6*\linewidth]{\texttuple{The funding}{will be delayed}{}};
    \node(c)[right=1 of C, text width=0.6*\linewidth]{\texttuple{Congress}{fail}{to increase [...]}};
    \node(d)[right=1 of D, text width=0.6*\linewidth]{\texttuple{President Bush}{fail}{to increase [...]}};

    \draw[solid, <->] (A)..controls +(west:6) and +(west:6)..([yshift=10]B) node [left, midway] () {Contrast};
    \draw[solid, ->] (B)..controls +(west:6) and +(west:6)..([yshift=5]C) node [left, midway] () {Condition};
    \draw[solid, ->] ([yshift=-10]B)..controls +(west:6) and +(west:6)..([yshift=-5]D) node [left, midway] () {Condition};
    \draw[solid, <->] ([yshift=-5]C)..controls +(west:5) and +(west:5)..([yshift=5]D) node [right, midway] () {List};

    \draw[solid, ->] (A) to (a);
    \draw[solid, ->] (B) to (b);
    \draw[solid, ->] (C) to (c);
    \draw[solid, ->] (D) to (d);

\end{tikzpicture}
\end{minipage}
\end{cminipage}

\vspace{0.2cm}
$\downarrow$
\vspace{0.2cm}

Output/RDF-Representation\\
\vspace{0.2cm}

\begin{minipage}{0.9\textwidth}
\centering

\begin{minipage}{0.6\textwidth}
\centering
\begin{tikzpicture}[scale=0.6, every node/.style={align=center, transform shape}]
\node[rectangle, solid, draw=black, minimum width=1.0*\linewidth, rounded corners=5pt]{
\begin{BVerbatim}
#1    0    the Treasury    will announce    details [...]
    S:TEMPORAL    on Monday
    L:CONTRAST    #2 

#2    0    the funding    will be delayed 
    L:CONTRAST     #1
    L:CONDITION    #3
    L:CONDITION    #4

#3    1    Congress    fail    to increase [...]
    L:LIST    #4

#4    1    president Bush    fail    to increase [...]
    L:LIST    #3
\end{BVerbatim}

};
\end{tikzpicture}
\end{minipage}%
\begin{minipage}{0.2\textwidth}
\centering
\begin{tikzpicture}[scale=0.5, every node/.style={align=center, transform shape}]
    \node(A) at (1, 3) [circle, solid, draw=black, text width=0.1*\columnwidth]{};
    \node(B) at (3, 3) [circle, solid, draw=black, text width=0.1*\columnwidth]{};
    \node(C) at (0, 1.5) [circle, solid, draw=black, text width=0.1*\columnwidth]{};
    \node(D) at (2, 1.5) [circle, solid, draw=black, text width=0.1*\columnwidth]{};
    \node(E) at (4, 1.5) [circle, solid, draw=black, text width=0.1*\columnwidth]{};
    \node(F) at (1, 0) [circle, solid, draw=black, text width=0.1*\columnwidth]{};
    \node(G) at (3, 0) [circle, solid, draw=black, text width=0.1*\columnwidth]{};
    \draw[solid, -] (A) to (B);
    \draw[solid, -] (C) to (D);
    \draw[solid, -] (B) to (D);
    \draw[solid, -] (B) to (E);
    \draw[solid, -] (D) to (F);
    \draw[solid, -] (F) to (G);
    \draw[solid, -] (D) to (G);
\end{tikzpicture}
\end{minipage}%
\end{minipage}%


\caption{Workflow for an example sentence}
\label{fig:workflow}
\end{figure}
